Reaction rates and transport in neutron stars

Understanding signals from neutron stars requires knowledge about the transport inside the star. We review the transport properties and the underlying reaction rates of dense hadronic and quark matter in the crust and the core of neutron stars and point out open problems and future directions.

==> crust_react.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reaction rates}\label{S:crust_reaction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Neutrino emission}\label{S:neutrino_emission_crust}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\com{Only a section plan at the moment}

Many reactions, as summarized in Ref.~\citet{Yakovlev2001physrep}.
The updated references are collected in
Ref.~\cite{Potekhin2015SSRv}. It seems, that we can be brief
here, may be emphasize the dominant reactions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Reactions in accreted
crust}\label{S:reactions_accretedcrust}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\com{Only a section plan at the moment}

Crust is set out of equilibrium on accretion. Various
nucleosynthesis reactions. Most important: deep crustal heating
reactions: electron captures; pycnonuclear reactions. Also Urca
cycles (Schatz Nature paper).

For deep crustal heating only energy output is really needed, not
rates.

The reaction rates are crucial when the reaction networks are
calculated. So for bursts and superbursts nucleosynthesis. We
cannot go in any details here, probably need to refer to recent
nuclear astrophysics reviews.

Deep crustal heating; Urca cycles. Discussion of superbursts.
Shallow heating. Ashes nucleosynthesis throughout the star. How to
come from high ${\cal Q}$ to low ${\cal Q}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Crustal cooling observations}\label{S:qxrt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\com{I put this in a separate section, since I strongly assume
that this should be covered by Degenaar and Poutannen, in which
case we can omit this (yet unwritten) section. }

\com{Only a section plan at the moment}

The observations of NS crust cooling are one of a few ways to
probe the physics of the crust. Essentially, the transport
properties (thermal conductivity) play crucial role here. Initial
thermal relaxation -- one of the possibilities. One need a
recently formed NS which can be observed with X-ray satellites.
Only possibility so far -- SN87A. Unfortunately, no CCO there
(possibly absorbed under the remnant shell; there are some hints
of the PWN-like emergence. But this will be disappointing since
then the pulsar behavior, hence non-thermal emission is present,
which will probably made impossible to observe the NS surface
temperature. Like the situation in Crab).

Fortunately -- another possibility exists: the Soft X-ray
transients.  Periodic episodes of accretion and cooling. Concept
of deep crustal heating: reactions induced in accreted star heats
it. Brief discussion of usual transients with application to
cooling can go to the end, or to the beginning -- it relates to
neutrino emission.

Here we focus on Quasi-persistent transients, where the crust is
dropped out of equilibrium with core an the subsequent cooling can
be observed (this was observed also in one (two?) normal
transients). Relation of these observations to transport:
 
\begin{equation}\label{eq:cooling_time}
\tau \propto \frac{C_V (\delta r)^2}{\kappa}
\end{equation}
 
 Thus the cooling
 reflects the thermal wave going from the interior and the
 cooling curve can be mapped to conductivity (and heat capacity)
 profile in the crust.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.7\textwidth, angle=-90]{fivetransients}
\caption{Crustal cooling observations for five quasi-persistent soft X-ray transients. The figure is reproduced from Ref.~\cite{Turlione2015A&A}}
\label{fig:SXRTs}
\end{center}
\end{figure}



What is established: relatively high conductivity; unknown shallow
source is mandatory; possible resistive layer in pasta (due to
Horowitz, but there can be purely observational explanantion -
Cackett).

How modelled - according to above, one parameterized the
conductivity in accreted with effective impurity parameter.
\com{the info from the block below may go to
Sec.~\ref{S:kincoeff_imp}}
 As discussed, this is valid
when the impurity parameter is not large and impurities are
uncorrelated. The situation in accreted crust is more challenging.
The  hydrogen-reach material accreted on the NS surface undergo
rp-process nucleosynthesis which leads to a diverse set of nuclei
e.g., \citep{Schatz2001PhRvL,Woosley2004ApJS}. \com{update refs.}
When the ashes of the hydrogen burning are buried deeper under
pressure of newly accreted material, the electron capture
reactions produce neutron rich nuclei. As the density and hence
$\Gamma$ parameter increases, the liquid solidifies \com{at larger
Gamma then OCP} and recent molecular dynamics simulations shows
that the phase separation occurs at this point, so that low-Z
elements remains in liquid phase, while high-Z elements are
immersed in the solid \citep{Horowitz2007PhRvE, Mckinven2016ApJ}.
The simulations  show that ${\cal Q}$ values in the liquid phase
near the crystallization point are about $30-50$, while in the
solid phase ${\cal Q}$ can be as low as $10$
\citep{Mckinven2016ApJ}.


Convection due to phase separation.

Mention some progress in multi $Q-imp$ modelling. What is really
probed (Brown\&Cumming)- the conductivity in the inner layers,
sine the outermost layers are dominated by the shallow source, and
this is another story. So in the picture of chemical separation
you probe the deeper parts where $Q$ may be smaller (and pasta).

The problem with superbursts: they need small conductivity. But in
outer layers. Some discussion from literature. Shallow heating
seems to help here also. Refer to Poutannen and Degenaar for
details.



\citet{Gupta2007ApJ,Gupta2008PhRvL,Steiner2012PhRvC,Mckinven2016ApJ}

Ashes. Accreted crust. Linear mixing rule and around it. Hybrid
crust.


Buried magnetic field.

Future developments for a crust: Robust description of a strongly
coupled system -- resolution of the discussion on the
melting-point transition; robust treatment of impurities;
superlattice; nature of the shallow source; electric conduction
and dissipation of the magnetar field: where, how fast, internal
heating (Kaminker) or external (Beloborodov).

